Morphic Sequences: Complexity and Decidability

In this work we recall Pansiot's result on the complexity of pure morphic sequences and we use the tools developed by Devyatov for morphic sequences to prove the decidability of the complexity class of pure morphic sequences.

==> eptcsdata.tex <==
\providecommand{\firstpage}{113}
\providecommand{\publicationstatus}{S. Brlek and L. Ferrari (Eds.): GASCom 2024\\
EPTCS 403, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.403.24}{10.4204/EPTCS.403.24}}

